The VoxCeleb Speaker Recognition Challenge: A Retrospective

The VoxCeleb Speaker Recognition Challenges (VoxSRC) were a series of challenges and workshops that ran annually from 2019 to 2023. The challenges primarily evaluated the tasks of speaker recognition and diarisation under various settings including: closed and open training data; as well as supervised, self-supervised, and semi-supervised training for domain adaptation. The challenges also provided publicly available training and evaluation datasets for each task and setting, with new test sets released each year. In this paper, we provide a review of these challenges that covers: what they explored; the methods developed by the challenge participants and how these evolved; and also the current state of the field for speaker verification and diarisation. We chart the progress in performance over the five installments of the challenge on a common evaluation dataset and provide a detailed analysis of how each year's special focus affected participants' performance. This paper is aimed both at researchers who want an overview of the speaker recognition and diarisation field, and also at challenge organisers who want to benefit from the successes and avoid the mistakes of the VoxSRC challenges. We end with a discussion of the current strengths of the field and open challenges. Project page : https://mm.kaist.ac.kr/datasets/voxceleb/voxsrc/workshop.html

==> Tables/valtest_stats.tex <==
\begin{table*}[!h]
\begin{center}
\caption{Statistics of validation and test sets. Entries in speaker verification tracks that have four values are reported as \# of utterances, \# of pairs, total \# of speakers and an average length of segment in seconds, while in speaker diarisation tracks the entries mean average \# of speakers per each audio, total \# of audio files and the average length of the audio file in seconds.}
\label{tab:valtest_stats}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cllll@{}}
\toprule
                     & \multicolumn{1}{c}{\textbf{Track 1}}                                                                                                    & \multicolumn{1}{c}{\textbf{Track 2}}                                                                                          & \multicolumn{1}{c}{\textbf{Track 3}}   &    \multicolumn{1}{c}{\textbf{Track 4}}                                                                                                                   \\ \midrule
\textbf{Task}        & \multicolumn{1}{c}{Speaker verification (Closed)}                                                                                       & \multicolumn{1}{c}{Speaker verification (Open)}                                                                               & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Self-supervised speaker verification (2020-2021)\\ / Semi-supervised domain adaptation (2022-2023)\end{tabular}}&\multicolumn{1}{c}{Speaker diarisation (Open)}  \\ \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}VoxSRC\\ 2019\end{tabular}}& \begin{tabular}[c]{@{}l@{}} Val :  4,715 / 37,720 / 40 / 8.3  \\ Test : 19,154 / 208,008 / 745 / 7.4\end{tabular}        & \begin{tabular}[c]{@{}l@{}} Val : 4,715 / 37,720 / 40 / 8.3 \\ Test : 19,154 / 208,008 / 745 / 7.4\end{tabular}          & -           &  -  \\ \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}VoxSRC\\ 2020\end{tabular}} & \begin{tabular}[c]{@{}l@{}} Val :  140,185 / 263,486 / 1,251 / 8.2\\ Test : 118,439 / 1,695,248 / 1,440 /  5.0\end{tabular} & \begin{tabular}[c]{@{}l@{}}Val :  140,185 / 263,486 / 1,251 / 8.2\\ Test : 118,439 / 1,695,248 / 1,440 / 5.0\end{tabular} & \begin{tabular}[c]{@{}l@{}} Val :  140,185 / 263,486 / 1,251 / 8.2\\ Test : 118,439 / 1,695,248 / 1,440 / 5.0\end{tabular} & \begin{tabular}[c]{@{}l@{}}Val :  4.5 / 216 / 338.2 \\ Test : 6.5 / 232 / 675.6\end{tabular}     \\ \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}VoxSRC\\ 2021\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Val : 64,711 / 60,000 / 1,251 / 8.1\\ Test : 116,984 / 476,224 / 1,440 / 5.0\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Val : 64,711 / 60,000 / 1,251 / 8.1\\ Test : 116,984 / 476,224 / 1,440 / 5.0\end{tabular}      & \begin{tabular}[c]{@{}l@{}} Val :  64,711 / 60,000 / 1,251 / 8.1\\ Test : 116,984 / 476,224 / 1,440 / 5.0\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Val :  5.5 / 448 / 512.9 \\ Test : 5.6 / 264 / 452.1\end{tabular}        \\ \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}VoxSRC\\ 2022\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Val : 110,366 / 305,196 / 2,307 / 8.4\\ Test : 34,684 / 317,973 / 1,974 / 7.4\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Val : 110,366 / 305,196 / 2,307 / 8.4\\ Test : 34,684 / 317,973 / 1,974 / 7.4\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Val :  2,400 / 40,000 / 120 / 9.4\\ Test : 18,377 / 30,000 / 56 / 9.1\end{tabular}              & \begin{tabular}[c]{@{}l@{}} Val :  5.5 / 448 / 512.9 \\ Test : 5.5 / 360 / 449.2\end{tabular}              \\ \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}VoxSRC\\ 2023\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Val : 63,516 / 49,987 / 2,140 / 8.2\\ Test : 256,547 / 825,437 / 2,532 / 5.3\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Val : 63,516 / 49,987 / 2,140 / 8.2\\ Test : 256,547 / 825,437 / 2,532 / 5.3\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Val :  2,400 / 40,000 / 120 / 9.4\\ Test : 21,997 / 80,000 / 56 / 8.9\end{tabular}              & \begin{tabular}[c]{@{}l@{}}Val :  5.5 / 448 / 512.9 \\ Test : 5.8 / 413 / 519.6 \end{tabular}              \\ \bottomrule
\end{tabular}}
\end{center}
\end{table*}
